JoinBoost: Grow Trees Over Normalized Data Using Only SQL

Although dominant for tabular data, ML libraries that train tree models over normalized databases (e.g., LightGBM, XGBoost) require the data to be denormalized as a single table, materialized, and exported. This process is not scalable, slow, and poses security risks. In-DB ML aims to train models within DBMSes to avoid data movement and provide data governance. Rather than modify a DBMS to support In-DB ML, is it possible to offer competitive tree training performance to specialized ML libraries...with only SQL? We present JoinBoost, a Python library that rewrites tree training algorithms over normalized databases into pure SQL. It is portable to any DBMS, offers performance competitive with specialized ML libraries, and scales with the underlying DBMS capabilities. JoinBoost extends prior work from both algorithmic and systems perspectives. Algorithmically, we support factorized gradient boosting, by updating the $Y$ variable to the residual in the non-materialized join result. Although this view update problem is generally ambiguous, we identify addition-to-multiplication preserving, the key property of variance semi-ring to support rmse, the most widely used criterion. System-wise, we identify residual updates as a performance bottleneck. Such overhead can be natively minimized on columnar DBMSes by creating a new column of residual values and adding it as a projection. We validate this with two implementations on DuckDB, with no or minimal modifications to its internals for portability. Our experiment shows that JoinBoost is 3x (1.1x) faster for random forests (gradient boosting) compared to LightGBM, and over an order magnitude faster than state-of-the-art In-DB ML systems. Further, JoinBoost scales well beyond LightGBM in terms of the # features, DB size (TPC-DS SF=1000), and join graph complexity (galaxy schemas).

==> sections/microexp.tex <==
\begin{figure*}
\centering
  \begin{subfigure}[t]{0.45\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/data_load.pdf}
      \caption{Data Load}
 \end{subfigure}
 \hfill
     \begin{subfigure}[t]{0.5\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/update.pdf}
      \caption{Update. DP is combination of DuckDB and Pandas.}
 \end{subfigure}
 \hfill
   \begin{subfigure}[t]{0.31\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/aggregation.pdf}
      \caption{Data Aggregation}
 \end{subfigure}
 \hfill
    \begin{subfigure}[t]{0.31\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/aggregation_thread.pdf}
      \caption{Aggregation diff threads}
 \end{subfigure}
 \hfill
    \begin{subfigure}[t]{0.31\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/agg_join.pdf}
      \caption{Aggregation-Join}
 \end{subfigure}
 \hfill
    \begin{subfigure}[t]{0.31\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/aggregation_pandas.pdf}
      \caption{Aggregation. Combination of DuckDB and Pandas slightly degrades performance.}
 \end{subfigure}
 \hfill
     \begin{subfigure}[t]{0.31\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/agg_join_pandas.pdf}
      \caption{Aggregation join. Combination of DuckDB and Pandas slightly degrades performance.}
 \end{subfigure}
 \hfill

\caption{Micro-Benchmarks for different systems.}
\end{figure*}

\section{Micro-benchmarks}

\begin{myitemize}
\item {\bf DBMS-X}: One of the most popular relational database management systems. Disk-based only. Could be column stored ({\bf X-col}) or row stored ({\bf X-row}). Annoymized due to DeWitt clause.
\item {\bf DuckDB~\cite{raasveldt2019duckdb}}: In-process SQL OLAP database management system. Column store only. Could be disk-based ({\bf D-disk}) or memory-based ({\bf D-mem}). Highly optimized.
\item {\bf Pandas}  Dataframe: In-memory only data structure. Stored column-wise. The internals are implemented in C. Highly efficient. Widely used for data analysis and machine learning. Pandas dataframes are single-thread only.
\item {\bf Dask}: Similar to Pandas but more efficient. We note that Dask does computation lazily including reading data from disk, which makes some of its queries unfairly slow. We study two approaches: lazily read file ({\bf Dask-Lazy}) or eagerly read data ({\bf Dask-Eager}) first as pandas Dataframe, then transform it to a dask DataFrame. Neither dominates so we report both.
\end{myitemize}

\noindent {\bf Testing Environment:} TODO system details. 8 cores. 100 GB memory. SSD.

\noindent {\bf Datasets:} We use synthetic dataset to control the variables. By default, we create a fact table with $|F| = 100M$ rows and one dimension tables with $|D| = 10K$ rows. The fact table has schema $[Dim, target]$. The target variable contains random integers. The dimension table has schema $[Dim, feature]$. The feature are a range variable from 1 to $|D|$ (for the update-select experiments as discussed below). Each dimension key maps to $|F|/|D| = 10K$ rows in fact table.

\noindent {\bf Workloads:} We consider the following workloads important for model training:

\begin{myitemize}
\item {\bf Data Load}: Loading data into the system is the first step. (Our assumption is that most datasets are already in database systems but likely not stored in memory. Therefore, loading data into memory is more interesting here.) We create the fact table and dimension table locally as csv files, and load them into different systems.

\item {\bf Aggregation}: Aggregation is needed to compute the best split. We test the performance of aggregation over fact table: $\gamma_{MAX(SUM)}(\gamma_{Dim, SUM(target)}(F))$, and vary the number of groupings $|D|$.

\item {\bf Join-Aggregation}: When computing the messages, we need to perform join-aggregation. We test the performance of materializing (as table) the aggregation over the join between the fact table and the dimension table: $\gamma_{feature, SUM(target)}(F \bowtie D)$,  and vary the number of groupings $|D|$. We further study the overhead of materialization.

\item {\bf Update from Select}: For gradient boosting, we need to update the residuals for the next round of boosting. This requires as to "Select" each leaf node and "Update" the residuals.  Number of clauses. Selectivity. Pandas loc or np.where. Semi-join vs filter.
\end{myitemize}

We note that, for current baselines, there are multiple ways to perform the workload. For instance, to update the table, we can either update in place using "set" clause, or create a new table with updated values. We have exhaustively experimented with different possible options and report the best one for each baseline.

\subsection{Data Load}

For databases, we create table for F and D. For Pandas, we create DataFrames.

\begin{itemize}
\item DBMS-X by default load data as row store, and is then converted into column store. DBMS-X has large data load overhead.

\item DuckDB is competitive to Pandas Dataframe.

\item Dask-L doesn't read the file as it is done lazily.

\end{itemize}




\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{images/gb_breakdown.pdf}
\caption{Final Breakdown of training one tree for Favorita, then update the residuals in the fact table. DP use Pandas DataFrame for efficient update. DP-para further exploits inter-query parallelism.}
\end{figure}

\subsection{Aggregation}

We compute $\gamma_{MAX(SUM)}(\gamma_{Dim, SUM(target)}(F))$ and vary the number of groupings $|Dim| = \{1, 100, 10K, 1M\}$.  

\begin{itemize}
\item For DBMS-X, row store is slow. Column store improves performance significantly.

\item Pandas is slower than databases because it has single thread. Dask-E uses multiple threads and is competitive.

\item Dask-L is slow as it also reads the file.

\end{itemize}



How much does thread matter? We vary the number of threads to $\{1,2,4,8\}$. We note that there is a diminishing return with respct to the number of threads.




\subsection{Join-Aggregation}
We compute $\gamma_{feature, SUM(target)}(F \bowtie D)$ and vary the number of groupings $|feature| = \{1, 100, 10K, 1M\}$. 


\begin{itemize}
\item Join operators from Pandas and Dask are slow. This is consistent with previous experiments \footnote{https://duckdb.org/2021/05/14/sql-on-pandas.html}.

\item For DBMS, column store improves join performance.

\end{itemize}



\subsection{Update}

The final step of gradient boosting is to update the residuals for each leaf node. We consider a decision stump that splits $feature$ by half.

We consider two types of leaf updates:

\begin{itemize}
\item {\bf Selection:} We apply the predicate over fact table to select leaf nodes, then update fact table.
The corresponding SQL for one leaf node is: {\it UPDATE fact SET target = new value WHERE dim < 5000}.

\item {\bf Semi-Join:} We apply the predicate over dim table, compute the message, then semi-join the message with fact.
The corresponding SQL is: {\it UPDATE fact SET target = new value WHERE dim in (SELECT dim FROM message)}.
\end{itemize}


We try different alternatives to update columns and report the best approach. For instance, we find that ”set” clause is prohibitively slow for DBMS-X, so we replace the table with a new table of updated values. For Pandas Dataframe, we use np.where which creates an updated column efficiently. For DBMS-X-col, the new table is first created as row store then converted into column store.

Takeaways:

\begin{itemize}
\item Pandas update is much faster than Databases.

\item Selection is slightly faster than Semi-join.
\end{itemize}

We find that the slow update is the key bottleneck for DBMS systems to perform well. This is expected as updating residuals is a new type of workload different to the traditional OLAP.


However, our initial attempt while improves the performance for disk-based DuckDB, the improvement is not that significant. After trial and error, we find that it is due to the slow semi-join between DuckDB table and Pandas DataFrame.
% for numerical computation like column wise addition, should use pandas as duckdb is slow
To avoid semi-join, we maintain the full join result and apply the predicate of leaf node directly. While materializing the full join result is against the original intention of factorized learning, we note that it is a temporal work around to the slow semi-join and can be removed in the future when DuckDB has better support.

Gradient boosting parallelism

Hard to exploit intra-query parallelism, as queries in gradient boosting are dependent and unbalanced.

We mainly exploit  types of inter-query parallelism:

\begin{itemize}
\item {\bf Parallelize Messages}: Messages from the fact table to dimension tables are independent yet expensive. We parallize messages.

\item {\bf Parallelize Tree Nodes}: Each Tree nodes use cjt to copy annotations from parent node, but the future queries are independent. We parallelize between tree nodes.

\item {\bf Parallelize Features Split}: For each tree node after calibration, we need to find the best split for each feature. These features are independent and could be parallelized. 

\item {\bf Parallelize Residual Updates}: During updates, we update the residual for the predication from each tree nodes. These updates could be parallelized.

\end{itemize}

We note that DuckDB support for inter-query parallelism is limited. For instance, DuckDB tables created by one threads are not visible to the other , and we work around this issue by storing messages as Pandas DataFrame. These issues force us to implement parallelism only for memory-based DuckDB and hurt the performance. As DuckDB is actively updated, we expect a better result when DuckDB supports better parallelism.

The final result is shown in the breakdown. DP-para reduce the time of DP by $28\%$



\begin{algorithm}

\DontPrintSemicolon

% Set Function Names
  \SetKwFunction{FSplit}{findBestSplit}
  \SetKwFunction{FTree}{buildTree}
  \SetKwFunction{FSub}{Sub}
 
% Write Function with word ``Function''
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FSplit {$R$}}{
        best\_score, best\_split = 0, None\;
        \ForEach{$A \in X$}{
            \ForEach{$\sigma$ over $A$}{
                cur\_score = eval($\sigma$, R)\;
                \If{cur\_score $>$ best\_score}{
                    best\_score, best\_split = cur\_score, $\sigma$\;
                }
            }
        }
        \KwRet best\_score, best\_split\;
  }
  \;

  \Fn{\FTree{$R, max\_leaves$}}{
    leafQueue = PriorityQueue()\;
    
    leafQueue.push(\FSplit(R))\;
    t = Tree()\;
    \While{leafQueue.isNotEmpty() and t.numLeaves() $<max\_leaves$ }{
        \_, $\sigma$ = leafQueue.pop()\;
        t.addLeaf($\sigma$)\;
        leafQueue.push(\FSplit($\sigma(R)$))\;
        leafQueue.push(\FSplit($\Bar{\sigma}(R)$))\;
    }
    \KwRet t\;
  }
  \caption{Tree-Based Model}
\end{algorithm}


==> sections/semijoinmsg.tex <==
\section{Semi-join Message}
\label{sec:semi_msg}

Consider the database with the fact table $F$ and other tables $D_1, \dots, D_n$, and message passing rooted at $F$. We use the following notations: $M(R)$ be the set of all incoming messages from $R$'s children, $J_{R, S}$ be the join key between $R$ and $S$. Since the join graph is acyclic, we may select the fact table as root and model the join graph as a tree. We use $p(D_i)$ to denote the parent of $D_i$ and $des(D_i)$ to denote the descendants of $D_i$. We would like to show $F \Join \pi_{S_F}(\sigma(D_1) \Join \dots \sigma(D_k)) = F \Join M(F)$. Consider a leaf table $D_\ell$ in the join graph, the message it sends to its parent is $\gamma_{J_{D_\ell, p(D_\ell)}}(\sigma(D_\ell))$. Suppose that for an internal node $D_i$ at level $k > 1$, the message it sends to its parent is 
$$\gamma_{J_{D_i, p(D_i)}}(\sigma(D_i)\Join\{\sigma(des(D_i))\})$$
Consider an internal node $D_j$ at level $k - 1$, the message it sends to its parent is
\begin{align*}
    &\text{ } \gamma_{J_{D_j, p(D_j)}} (\sigma(D_j) \Join M(D_j))\\
    = & \gamma_{J_{D_j, p(D_j)}} (\sigma(D_j) \Join \{\gamma_{J_{D_p, D_j}}(\sigma(D_p)\Join\{\sigma(des(D_p))\}) \ | \ p(D_p) = D_j\}) \text{ expansion}\\
    = & \gamma_{J_{D_j, p(D_j)}} (\sigma(D_j) \Join \{\sigma(D_p)\Join\{\sigma(des(D_p))\} \ | \ p(D_p) = D_j\})\text{ aggregation pushup}\\
    = & \gamma_{J_{D_j, p(D_j)}} (\sigma(D_j) \Join \{\sigma(des(D_j))\}) \text{ definition of descendants}
\end{align*}
Thus, it follows that 
\begin{align*}
    &\text{ } F \Join \pi_{S_F}(\sigma(D_1) \Join \dots \sigma(D_k)) \\
    &= F \Join \{\gamma_{D_i, F}(\sigma(D_i) \Join \{\sigma(des(D_i)\}) \ | \ p(D_i) = F\} \text{ partition of subtree rooted at children of } F \\
    &= F \Join M(F) \text{ substitution}
\end{align*}

\noindent For each leaf $i$ in the decision tree, we may denote the set of predicates from the root to $i$ with $\sigma_i$. We have shown that $F \Join \pi_{S_F}(\sigma_i(D_1) \Join \dots \sigma_i(D_k)) = F \Join M(F)$. This means that each $\sigma_i$ selects the same tuples in $F$ as joining messages with $F$ in leaf $i$.
Based on the definition of $U$, selecting tuples in $F$ using $U$ is equivalent to semi-join $F$ with incoming messages from each leaf.
